Qabas: An Open-Source Arabic Lexicographic Database

We present Qabas, a novel open-source Arabic lexicon designed for NLP applications. The novelty of Qabas lies in its synthesis of 110 lexicons. Specifically, Qabas lexical entries (lemmas) are assembled by linking lemmas from 110 lexicons. Furthermore, Qabas lemmas are also linked to 12 morphologically annotated corpora (about 2M tokens), making it the first Arabic lexicon to be linked to lexicons and corpora. Qabas was developed semi-automatically, utilizing a mapping framework and a web-based tool. Compared with other lexicons, Qabas stands as the most extensive Arabic lexicon, encompassing about 58K lemmas (45K nominal lemmas, 12.5K verbal lemmas, and 473 functional-word lemmas). Qabas is open-source and accessible online at https://sina.birzeit.edu/qabas.

==> lemma_linking.tex <==
\subsection{Auto Mapping}
\label{sec:auto-mapping}

To facilitate the process of lemma selection, we adopted lemmas automatically by initially adopting all lemmas from the 'Modern' dictionary \citep{}, followed by adopting all lemmas from the 'SAMA' database \citep{} and subsequently adopting lemmas from 150 other dictionaries. Each lemma that was adopted had all its information transferred along with it, including details such as number, gender, root, voice, transitivity, augmentation, part of speech, and POS category.

Moreover, each lemma underwent a mapping procedure with similar lemmas from the other dictionaries, employing a semi-automatic approach. Initially, we established rules for mapping lexicons with one another.  In essence, to map the lemma \Ar{يَوْميٌّ} across the SAMA, Modern, and Ghani lexicons, considering its noun classification, we created distinct sets for each form:

SAMA:
Singulars: \{"\Ar{يَوْمِيَّة}"\} 
Duals: \{"\Ar{يَوْمِيَّتَي}", "\Ar{يَوْمِيَّتان}", "\Ar{يَوْمِيَّتا}", "\Ar{يَوْمِيَّتَيْن}"\}
Plurals: \{"\Ar{يَوْمِيّا}", "\Ar{يَوْمِيَّي}", "\Ar{يَوْمِيّان}", "\Ar{يَوْمِيَّيْن}"\}
Root: \{-\}

Modern:
Singulars: \{"\Ar{يَوْميّ}"\}
Duals: \{-\}
Plurals: \{-\}
Root: \{"\Ar{ي و م}"\}

Ghani:
Singulars: \{"\Ar{يَوْمِيٌّ}", "\Ar{يَوْمِيّةٌ}"\}
Duals: \{-\}
Plurals: \{-\}
Root: \{"\Ar{ي و م}"\}

Consequently, it was observed that the singular set in Modern is a subset of the singular set in Ghani, and since the roots were identical, the Modern lemma was successfully mapped with the Ghani lemma. Additionally, the lemma was mapped between Ghani and SAMA.

Similarly, a comparable rule was applied to verbs, with a focus on past verbs, present forms, and CV patterns. This mapping process encompassed approximately 80\% of the Qabas dataset.

Following this automated mapping, linguists conducted a meticulous manual verification using a dedicated tool, designed to facilitate necessary adjustments to the lemmas. Subsequently, they addressed the remaining mappings that could not be mapped automatically.


Subsequently, linguists manually verified this automatic mapping using a tool that was developed and constructed to assist linguists in making necessary adjustments to the lemmas.

However, it's important to note that this linking process does not block the addition of manually inserted lemmas, such as the dialect lemmas.

\subsection{Mapping Framework}
The objective of this framework is to establish semantic links between lexical senses in various linguistic resources through a mapping correspondence. 

Definition: In the context of this framework, a mapping correspondence between two lemmas, denoted as lem1 and lem2, is defined as follows:

<lem1, lem2, R, P>

Where:

\begin{itemize}
    \item lem1 and lem2 represent the lemmas being mapped. 
    \item R signifies the mapping relationship between lem1 and lem2, which can take values like \Ar{نفسها: جميع التصريفات وجميع المعاني}...etc .
    \item P represents the precision percentage.
\end{itemize}

Each relationship is associated with a specific percentage. Table \ref{tab:relations_percentage} provides an overview of these relationships and the corresponding precision values. For instance, when we have <lemma1, lemma2, \Ar{نفسها جميع التصريفات جميع المعاني}>, it implies that lemma1 and lemma2 share an exact correspondence of 100\%, and so on.

In other words, precision refers to the degree to which the mapper (whether human or software) realizes a relationship between the first lemma and the second lemma, such as a "\Ar{نفسها جميع التصريفات جميع المعاني}" relationship. While this interpretation might align with set-theoretic semantics, implying, for example, that 100\% of the extensions of two lemmas are identical, these conceptualizations serve as valuable methodological tools for potentially excluding less certain or questionable mappings.

\begin{table}[]
\centering
\caption{relations\_percentage}
\label{tab:relations_percentage}
\begin{tabular}{|r|r|}
\hline
\multicolumn{1}{|c|}{Relation} & \multicolumn{1}{|c|}{Prec} \\ \hline
 \Ar{نفسها: جميع التصريفات وجميع المعاني} & 100\% \\ \hline
 \Ar{نفسها: جميع التصريفات وجميع المعاني، مفرد جمع} & 90\% \\ \hline
 \Ar{نفسها: جميع التصريفات وجميع المعاني، مفرد مثنى} & 80\% \\ \hline
 \Ar{نفسها: جميع التصريفات وجميع المعاني، مذكر مؤنث} & 70\% \\ \hline
 \Ar{نفسها: جميع التصريفات وجميع المعاني واختلاف الحالة الإعرابية} & 60\% \\ \hline
\Ar{نفسها: جميع التصريفات بعض المعاني} & 50\% \\ \hline
 \Ar{نفسها: بمعنى اسم العلم} & 40\% \\ \hline
% \Ar{مختلفة لفظا: بنفس المعنى} & 50\% \\ \hline
 \Ar{مختلفة: نفس المعاني} & 30\% \\ \hline
 \Ar{مختلفة: ترادف بعض المعاني}  & 20\% \\ \hline
 \Ar{مختلفة:علاقة اشتقاقية فيها إحالة للمعاني} & 10\% \\ \hline
\end{tabular}
\end{table}

This framework is employed for mapping lemmas in the Qabas dictionary to other dictionaries. Qabas has been fully mapped with Modern and Sama, and partially mapped with Ghani and other dictionaries. Qabas contains about 57K lexical senses sourced from numerous Arabic dictionaries. The mapping process was automated, and the relationship used is \Ar{نفسها الياً} (meaning "same automatically"). Subsequently, the lexicographers reviewed the automated mappings and modified this relationship to be one of the relations listed in Table \ref{tab:relations_percentage}. \\
Table \ref{tab:relations_counts} provides statistics regarding the mapping process and indicates which mapping relationships were utilized.


\begin{table}[]
\centering
\caption{relations\_percentage}
\label{tab:relations_counts}
\begin{tabular}{|r|r|}
\hline
\multicolumn{1}{|c|}{Relation} & \multicolumn{1}{|c|}{Counts} \\ \hline  
 \Ar{نفسها: جميع التصريفات وجميع المعاني} & 55380\\ \hline
 \Ar{نفسها: جميع التصريفات وجميع المعاني، مفرد جمع} & 1157 \\ \hline
 \Ar{نفسها: جميع التصريفات وجميع المعاني، مفرد مثنى} & 41 \\ \hline
 \Ar{نفسها: جميع التصريفات وجميع المعاني، مذكر مؤنث} & 889 \\ \hline
 \Ar{نفسها: جميع التصريفات وجميع المعاني واختلاف الحالة الإعرابية} & 207 \\ \hline
 \Ar{مختلفة لفظا: بنفس المعنى} & 1563 \\ \hline
 \Ar{مختلفة: نفس المعاني} & 692 \\ \hline
 \Ar{مختلفة: ترادف بعض المعاني} & 580 \\ \hline
 \Ar{نفسها: جميع التصريفات بعض المعاني} & 3846 \\ \hline
 \Ar{نفسها: بمعنى اسم العلم} & 1560 \\ \hline
 \Ar{مختلفة:علاقة اشتقاقية فيها إحالة للمعاني} & 93 \\ \hline
\end{tabular}
\end{table}



% \subsection{Statistics}
% Qabas contains about 57K lemmas, with 32K sourced from 'Modern' \citep{} – a substantial part of Qabas, because, we initially adopted the Modern Arabic language dictionary. This choice was made due to our belief that it is the closest to the modern lexicographic industry. The table below provides a detailed breakdown of lemma counts within each dictionary, as well as the number of lemmas linked to the Qabas lexicon. \\
% The Qabas lemmas are categorized into three groups, namely nouns, verbs, and functional words, with the following distribution: 44K nouns, 13K verbs, and 400 functional words. \\ 
